Eliciting and Understanding Cross-Task Skills with Task-Level Mixture-of-Experts

Recent works suggest that transformer models are capable of multi-tasking on diverse NLP tasks and adapting to new tasks efficiently. However, the potential of these multi-task models may be limited as they use the same set of parameters for all tasks. In contrast, humans tackle tasks in a more flexible way, by making proper presumptions on what skills and knowledge are relevant and executing only the necessary computations. Inspired by this, we propose to use task-level mixture-of-expert models, which has a collection of transformer layers (i.e., experts) and a router component that chooses from these experts dynamically and flexibly. We find that these models help improve the average performance gain (ARG) metric by 2.6% when adapting to unseen tasks in the few-shot setting and by 5.6% in the zero-shot generalization setting. Further, we show that the learned routing decisions partly rediscover human categorization of NLP tasks -- certain experts are strongly associated with extractive tasks, some with classification tasks, and some with tasks requiring world knowledge.

==> tables/hand_feature_desc.tex <==
\begin{table}[h]
\centering
\scalebox{0.8}{
\begin{tabular}{lp{15cm}}
\toprule
\textbf{Name}       & \textbf{Description}                                                                          \\\midrule
Extractive          & Output is copied and pasted from the input. (Output is a substring of the input)              \\
Linguistic          & Tasks focusing on grammatical correctness, semantic equivalence and linguistic phenomenon.    \\
Commonsense         & Tasks testing commonsense knowledge and commonsense reasoning capabilities                    \\
Co-reference        & Tasks requiring co-reference resolution                                                       \\
World Knowledge     & Tasks requiring world knowledge (acquired during pre-training)                                \\
Multi-hop           & Multi-step reasoning                                                                          \\
Sentence Completion & Requires the model to fill in a blank in the input or continue to generate based on the input \\
Synthesis           & Combining ideas and allowing an evolving understanding of text \href{https://beyondpenguins.ehe.osu.edu/issue/climate-change-and-the-polar-regions/summarizing-and-synthesizing-whats-the-difference}{(reference)}                           \\ \bottomrule    
\end{tabular}
}
\caption{Description of task features about high-level skills and others.}\label{tab:hand_feature_desc}
\end{table}
